KPQA: A Metric for Generative Question Answering Using Keyphrase Weights

In the automatic evaluation of generative question answering (GenQA) systems, it is difficult to assess the correctness of generated answers due to the free-form of the answer. Especially, widely used n-gram similarity metrics often fail to discriminate the incorrect answers since they equally consider all of the tokens. To alleviate this problem, we propose KPQA-metric, a new metric for evaluating the correctness of GenQA. Specifically, our new metric assigns different weights to each token via keyphrase prediction, thereby judging whether a generated answer sentence captures the key meaning of the reference answer. To evaluate our metric, we create high-quality human judgments of correctness on two GenQA datasets. Using our human-evaluation datasets, we show that our proposed metric has a significantly higher correlation with human judgments than existing metrics. The code is available at https://github.com/hwanheelee1993/KPQA.

==> table_nrqa_semeval.tex <==
\begin{table}[!t]
\footnotesize
\centering
\begin{tabular}
{L{0.34\columnwidth}C{0.1\columnwidth}C{0.1\columnwidth}C{0.11\columnwidth}C{0.1\columnwidth}}
\toprule

\multicolumn{1}{c}{\textbf{Metric}} & \multicolumn{2}{c}{\textbf{NarrativeQA}} &
\multicolumn{2}{c}{\textbf{SemEval}}\\ 

\cmidrule{2-5}
              & \textbf{$r$} & \textbf{$\rho$} 
              & \textbf{$r$} & \textbf{$\rho$}\\
\midrule

\textbf{BLEU-1} & 0.634 & 0.643 & 0.359 & 0.452 \\
\textbf{BLEU-4} & 0.258 & 0.570 & -0.035 & 0.439 \\
\textbf{ROUGE-L} & 0.707 & 0.708 & 0.566 & 0.580 \\
\textbf{METEOR} & 0.735 & 0.755 & 0.543 & 0.645 \\
\textbf{CIDEr} & 0.648 & 0.710 & 0.429 & 0.595 \\
\textbf{BERTScore} & \textbf{0.785} & 0.767 & 0.630 & 0.602 \\
\midrule
\textbf{BLEU-1-KPQA} & 0.709 & 0.692 & 0.358 & 0.47 \\
\textbf{ROUGE-L-KPQA} & 0.767 & 0.746 & 0.729 & 0.675 \\
\textbf{BERTScore-KPQA} & 0.783 & \textbf{0.769} & \textbf{0.748} & \textbf{0.677} \\

\bottomrule 
\end{tabular}
\caption{
Pearson Correlation($r$), Spearman's Correlation($\rho$) between various automatic metrics and human judgments of correctness for NarrativeQA dataset and SemEval 2018 Task 11 dataset. All of the results are statistically significant (p-value $<$ 0.01). %We use the dataset released from~\cite{chen2019evaluating}. 
}
\label{comparison-nrqa-semeval}
\end{table}


% Older Version SQuAD + FSVQA
\begin{comment}
\textbf{BLEU-1*} & 0.634 & 0.617 & 0.359 & 0.443\\ 
%\textbf{BLEU-4*} & 0.258 & 0.563 & -0.035 & 0.437\\
\textbf{ROUGE-L*} & 0.707 & 0.707 & 0.566 & 0.577\\
\textbf{METEOR*} & 0.734 & 0.752 & 0.543 & 0.642\\ 
%\textbf{BERTScore*} & 0.785 & 0.767 & 0.630 & 0.602\\
\textbf{BERTScore} & 0.785 & 0.767 & 0.630 & 0.602\\
\midrule
\textbf{BLEU-1-KPQA} & 0.702 & 0.715 & 0.389 & 0.536 \\ 
\textbf{ROUGE-L-KPQA} & 0.762 & 0.769 & \textbf{0.772} & \textbf{0.705} \\
\textbf{BERTScore-KPQA} & \textbf{0.790} & \textbf{0.770} & 0.738 & 0.626\\ 
\end{comment}
